WDD: Weighted Delta Debugging

Delta Debugging is a widely used family of algorithms (e.g., ddmin and ProbDD) to automatically minimize bug-triggering test inputs, thus to facilitate debugging. It takes a list of elements with each element representing a fragment of the test input, systematically partitions the list at different granularities, identifies and deletes bug-irrelevant partitions. Prior delta debugging algorithms assume there are no differences among the elements in the list, and thus treat them uniformly during partitioning. However, in practice, this assumption usually does not hold, because the size (referred to as weight) of the fragment represented by each element can vary significantly. For example, a single element representing 50% of the test input is much more likely to be bug-relevant than elements representing only 1%. This assumption inevitably impairs the efficiency or even effectiveness of these delta debugging algorithms. This paper proposes Weighted Delta Debugging (WDD), a novel concept to help prior delta debugging algorithms overcome the limitation mentioned above. The key insight of WDD is to assign each element in the list a weight according to its size, and distinguish different elements based on their weights during partitioning. We designed two new minimization algorithms, Wddmin and WProbDD, by applying WDD to ddmin and ProbDD respectively. We extensively evaluated Wddmin and WProbDD in two representative applications, HDD and Perses, on 62 benchmarks across two languages. The results strongly demonstrate the value of WDD. We firmly believe that WDD opens up a new dimension to improve test input minimization techniques.

==> approach.tex <==
In this section, we describe the workflow of our
approaches, \ie, \wdd and \wprobdd.
The analysis of the properties of our approaches,
\eg, efficiency and minimality, is also presented.

\input{approach-wdd}


\input{approach-wprobdd}



==> casestudies.tex <==



==> data_availability.tex <==
For replication, we have implemented \wddmin and \wprobdd and released
them publicly~\cite{zhang2024lprartifact}. \zxt{TODO: change the bib}


==> future_work.tex <==
\cn{No need to write future work in academic papers. Just remove this paragraph.}

Most existing delta debugging algorithms fail to consider
the specific characteristics of elements in the input list.
Besides, advanced minimization techniques integrate delta
debugging algorithms directly for their domain-specific minimization tasks.
In this paper, we argue that the features of elements should be
considered during delta debugging, and realize this idea in two
representative delta debugging algorithms, \ie, \ddmin and \probdd.
Since \ddmin and \probdd are designed with generality to work for any input,
the main feature that we can extract is the size of the elements.
However, for many language-specific techniques discussed in\cref{subsec:program_reduction},
the information of the elements can be significantly more detailed.
For example, in ddSMT~\cite{niemetz2013ddsmt},
it is possible to design tailored delta debugging strategies for
specific statements of SMT-LIBv2.
Therefore, extending our insight to leverage the unique characteristics
of these techniques presents a valuable avenue for future research.


==> tables/dd-example.tex <==
\begin{table}[]
    \centering
    \setlength{\tabcolsep}{2pt}
    \caption{}
    \label{tab:ddmin-example}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|*{1}{>{\centering\arraybackslash}m{0.05\columnwidth}}*{9}{>{\centering\arraybackslash}m{0.05\columnwidth}}|*{10}{>{\centering\arraybackslash}m{0.05\columnwidth}}|*{9}{>{\centering\arraybackslash}m{0.05\columnwidth}}|>{\centering\arraybackslash}m{0.05\columnwidth}|}
    \hline
    \multicolumn{10}{|c|}{ddmin}                                                                                                                                                                                                                                                                                                                                                                                                         & \multicolumn{10}{c|}{ProbDD}                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
    \multicolumn{1}{|c|}{1}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4} & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{1}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{2}                            & \multicolumn{1}{c|}{3}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5}    & \multicolumn{1}{c|}{6}                            & \multicolumn{1}{c|}{7}                            & \multicolumn{1}{c|}{8}                            & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{2}  & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{0.2}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.3}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.3}  & \multicolumn{1}{c|}{0.2}                          & \multicolumn{1}{c|}{0.2}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.3}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.3}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.3}  &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{3}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2} & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{2}  & \multicolumn{1}{c|}{1}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3}    & \multicolumn{1}{c|}{4}                            & \multicolumn{1}{c|}{5}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8}    & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{4}  & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4} & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.41} & \multicolumn{1}{c|}{0.3}                          & \multicolumn{1}{c|}{0.3}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.41} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.41} & \multicolumn{1}{c|}{0.3}                          & \multicolumn{1}{c|}{0.3}                          & \multicolumn{1}{c|}{0.3}                          &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{5}  & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{3}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2}    & \multicolumn{1}{c|}{3}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5}    & \multicolumn{1}{c|}{6}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{8}                            & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{6}  & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{0.41}                         & \multicolumn{1}{c|}{0.3}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.46} & \multicolumn{1}{c|}{0.41}                         & \multicolumn{1}{c|}{0.41}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.46} & \multicolumn{1}{c|}{0.3}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.46} &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{7}  & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{4}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{2}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6}    & \multicolumn{1}{c|}{7}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8}    & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{8}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2} & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{0.41}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.59} & \multicolumn{1}{c|}{0.46}                         & \multicolumn{1}{c|}{0.41}                         & \multicolumn{1}{c|}{0.41}                         & \multicolumn{1}{c|}{0.46}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.59} & \multicolumn{1}{c|}{0.46}                         &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{9}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4} & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{5}  & \multicolumn{1}{c|}{1}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4}    & \multicolumn{1}{c|}{5}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8}    & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{10} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.63} & \multicolumn{1}{c|}{0.59}                         & \multicolumn{1}{c|}{0.46}                         & \multicolumn{1}{c|}{0.41}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.63} & \multicolumn{1}{c|}{0.46}                         & \multicolumn{1}{c|}{0.59}                         & \multicolumn{1}{c|}{0.46}                         &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{11} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{6}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2}    & \multicolumn{1}{c|}{3}                            & \multicolumn{1}{c|}{4}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8}    & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{12} & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2} & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{0.63}                         & \multicolumn{1}{c|}{0.59}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.67} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.60} & \multicolumn{1}{c|}{0.63}                         & \multicolumn{1}{c|}{0.46}                         & \multicolumn{1}{c|}{0.59}                         & \multicolumn{1}{c|}{0.46}                         &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{13} & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{7}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5}    & \multicolumn{1}{c|}{6}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{8}                            & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{14} & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4} & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{0.63}                         & \multicolumn{1}{c|}{0.59}                         & \multicolumn{1}{c|}{0.67}                         & \multicolumn{1}{c|}{0.60}                         & \multicolumn{1}{c|}{0.63}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.65} & \multicolumn{1}{c|}{0.59}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0.65} &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{15} & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6}    & \multicolumn{1}{c|}{7}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8}    & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{16} & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{0.63}                         & \multicolumn{1}{c|}{0.59}                         & \multicolumn{1}{c|}{0.67}                         & \multicolumn{1}{c|}{0.60}                         & \multicolumn{1}{c|}{0.63}                         & \multicolumn{1}{c|}{0.65}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}1.00} & \multicolumn{1}{c|}{0.65}                         &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{17} & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{9}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{2}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8}    & T \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{18} & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{2}                         & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{4}                         & \multicolumn{1}{c|}{5}                         & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{0.63}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0}    & \multicolumn{1}{c|}{0.67}                         & \multicolumn{1}{c|}{0.60}                         & \multicolumn{1}{c|}{0.63}                         & \multicolumn{1}{c|}{0.65}                         & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{0.65}                         &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{19} & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}2} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3}    & \multicolumn{1}{c|}{4}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8}    & T \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{20} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & T & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{0.63}                         & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{0.67}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0}    & \multicolumn{1}{c|}{0.63}                         & \multicolumn{1}{c|}{0.65}                         & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{0.65}                         &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{21} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}  & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}4} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{11} & \multicolumn{1}{c|}{1}                            & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3}    & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8}    & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{22} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & T & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}1.00} & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{0.67}                         & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{0.63}                         & \multicolumn{1}{c|}{0.65}                         & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{0.65}                         &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{23} & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{12} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3}    & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}     & \multicolumn{1}{c|}{5}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8}    & T \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{24} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}  & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}5} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{0.67}                         & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}0}    & \multicolumn{1}{c|}{0.65}                         & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{0.65}                         &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{25} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}  & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 5}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & T & \multicolumn{1}{c|}{13} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3}    & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}     & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 5}}     & \multicolumn{1}{c|}{6}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8}    & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{26} & \multicolumn{1}{c|}{1}                         & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}  & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 5}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{0.67}                         & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}1.00} & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{0.65}                         &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{27} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}  & \multicolumn{1}{c|}{3}                         & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}  & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 5}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{14} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3}    & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}     & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 5}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{8}                            & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{28} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}  & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 5}}  & \multicolumn{1}{c|}{6}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{0.67}                         & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}1.00} &   \\ \cline{2-10} \cline{12-20}
    \multicolumn{1}{|c|}{29} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}  & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 5}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{7}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8} & F & \multicolumn{1}{c|}{15} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1}    & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}     & \multicolumn{1}{c|}{3}                            & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}     & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 5}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}8}    & F \\ \cline{2-10} \cline{12-19}
    \multicolumn{1}{|c|}{30} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}1} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 2}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}3} & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 4}}  & \multicolumn{1}{c|}{{\color[HTML]{C0C0C0} 5}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}6} & \multicolumn{1}{c|}{\cellcolor[HTML]{DAE8FC}7} & \multicolumn{1}{c|}{8}                         & F & \multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFC9E}1.00} & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{0}                            & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{1.00}                         & \multicolumn{1}{c|}{1.00}                         &   \\ \hline
    \end{tabular}%
    }
    \end{table}




